Learning Causal Alignment for Reliable Disease Diagnosis

Aligning the decision-making process of machine learning algorithms with that of experienced radiologists is crucial for reliable diagnosis. While existing methods have attempted to align their diagnosis behaviors to those of radiologists reflected in the training data, this alignment is primarily associational rather than causal, resulting in pseudo-correlations that may not transfer well. In this paper, we propose a causality-based alignment framework towards aligning the model's decision process with that of experts. Specifically, we first employ counterfactual generation to identify the causal chain of model decisions. To align this causal chain with that of experts, we propose a causal alignment loss that enforces the model to focus on causal factors underlying each decision step in the whole causal chain. To optimize this loss that involves the counterfactual generator as an implicit function of the model's parameters, we employ the implicit function theorem equipped with the conjugate gradient method for efficient estimation. We demonstrate the effectiveness of our method on two medical diagnosis applications, showcasing faithful alignment to radiologists.

==> para/abstract.tex <==
\begin{abstract}
    Aligning the decision-making process of machine learning algorithms with that of experienced radiologists is crucial for reliable diagnosis. While existing methods have attempted to mimic the behavior of radiologists reflected in the training data, they often suffer from the issue of learning pseudo-correlation. This is because their alignment is only associational, rather than causal. In this paper, we propose a causality-based alignment framework towards aligning the model's decision process with that of experts. Our key idea is to learn the causal decision chain employed by radiologists. To achieve this, we first identify the causal chain of model decisions via counterfactual generation. Then, we propose a causal alignment loss to ensure the identified chain aligned with that of radiologists. To optimize this loss that involves an implicit function of the model's parameters, we employ the implicit function theorem equipped with the conjugate gradient method for efficient estimation. We demonstrate the effectiveness of our method on two medical diagnosis applications, showcasing faithful alignment to radiologists.
\end{abstract}

==> para/abstract_xw_v1.tex <==
\begin{abstract}
    Aligning the decision-making process of machine learning algorithms with that of experienced radiologists is crucial for reliable diagnosis. While existing methods have attempted to align their prediction behavior to that of radiologists reflected in the training data, this alignment is primarily associational rather than causal, resulting in pseudo-correlation that may not transfer well. In this paper, we propose a causality-based alignment framework towards aligning the model's decision process with that of experts. Specifically, we first employ counterfactual generation to identify the causal chain of model decisions. To align this causal chain with that of experts, we propose a causal alignment loss that enforces the counterfactual generator for this model to focus on causal factors underlying each decision step in the whole prediction procedure. To optimize this loss that involves the counterfactual generator as an implicit function of the model's parameters, we employ the implicit function theorem equipped with the conjugate gradient method for efficient estimation. We demonstrate the effectiveness of our method on two medical diagnosis applications, showcasing faithful alignment to radiologists.
\end{abstract}

% %Our key idea is to learn the causal decision chain employed by radiologists. To achieve this, we first identify the causal chain of model decisions via counterfactual generation. Then, we propose a causal alignment loss to ensure the identified chain aligned with that of radiologists. 


==> para/experiment.tex <==
\section{Experiment}

In this section, we apply our method to two medical imaging diagnosis tasks: the benign/malignant classification of lung nodules and breast masses\footnote{We consider more diagnosis tasks and data modalities in Appx.~\ref{appx.more-modalities}.}. 

\subsection{Experimental Setups}

\textbf{Datasets \& Preprocessing.} We consider the LIDC-IDRI dataset \cite{armato2011lung} for lung nodule classification and the CBIS-DDSM dataset \cite{lee2017curated} for breast mass classification. 

The \emph{LIDC-IDRI} dataset contains thoracic CT images, each associated with bounding boxes indicating the nodule areas, a malignancy score ranging from $1$ to $5$, and six radiologist-annotated attributes (subtlety, calcification, margin, speculation, lobulation, and texture). Before analysis, we preprocess the images by resampling the pixel space and normalizing the intensity. For training and evaluation, we use the entire 2D slice as input, without explicitly cropping the nodule. We label those images with malignancy scores of $1$-$3$ as benign ($y=0$) and those with scores of $4$-$5$ as malignant ($y=1$). We split the dataset into training ($n=731$), validation ($n=238$), and test ($n=244$) sets.

The \emph{CBIS-DDSM} dataset contains breast mammography images with fine-grained annotations (mass bounding boxes, malignancy, and radiologist-annotated attributes). We preprocess the images by removing the background and normalizing the intensity. During training and evaluation, we randomly crop $250$ pixels around each mass and use the cropped image as input. We use the provided binary malignancy label and six annotated attributes (subtlety, shape, circumscription, obscuration, ill-definiteness, and spiculation). We follow the official dataset split, with $691$ masses in the training set and $200$ masses in the test set.

To test the ability of our method to learn expert-aligned features, we add a ``$+$"/``$-$" symbol on the top-left corner of each image as a spuriously correlated feature. This symbol coincides with the malignancy label in the training set, where images with $y=1$ are labeled with ``$+$" and those with $y=0$ are labeled with ``$-$"; but are assigned randomly in the validation and test sets. A well-aligned model should focus on the radiologist-annotated areas rather than the symbol.

\textbf{Evaluation Metrics.} To assess the alignment of our model relative to radiologists, we compute the Class Activation Mapping (CAM) \cite{selvaraju2017grad} and report its precision relative to the annotated areas, \emph{i.e.}, $\frac{\text{Area of (CAM} \, \cap \, {\text{Anno)}}}{\text{Area of CAM}}$. We also report the overall classification accuracy.

\textbf{Implementation Details.} We use the Adam optimizer, with a learning rate of $0.001$. We parameterize the attributes prediction network $f_{\theta_1}$ with a seven-layer Convolutional Neural Network (CNN), and train it for $100$ epochs with a batch size of $128$ for each iteration. For the classification network $f_{\theta_2}$, we parameterize it with a two-layer Multi-Layer Perceptron (MLP), and train it for $30$ epochs with a batch size of $128$. Please refer to Appx.~\ref{appx.network-arch} for details of the network architectures. For both networks, we train the cross-entropy loss $\mathcal{L}_{\text{cls}}$ and the alignment loss $\mathcal{L}_{\text{align}}$ in an alternating manner. For the hyperparameters $\alpha_1$ in Eq.~\ref{eq.counter-image-2} and $\alpha_2$ in Eq.~\ref{eq.counter-attribute}, we set them to $\alpha_1=0.01, \alpha_2=0.0005$ for LIDC-IDRI and $\alpha_1=0.07, \alpha_2=0.0005$ for CBIS-DDSM. For both datasets, we set $\beta_1=\beta_2=1$. We follow the $\mathrm{TorchOpt}$ \cite{ren2022torchopt} package to implement the conjugate gradient estimator. 


\subsection{Comparison with Baselines}

\textbf{Compared Baselines.} We compare our method with the following baselines: \textbf{i) \cite{ross2017right}} that achieved interpretability by penalizing the input gradient to be small in object-irrelevant areas; \textbf{ii) ICNN} \cite{zhang2018interpretable} that modified traditional CNN with an interpretable convolution layer to enforce object-centered representations; \textbf{iii) BagNet} \cite{brendel2019approximating} that approximated CNN with white-box bag-of-features models; \textbf{iv) \cite{rieger2020interpretations}} that required the model to produce a classification as well as an explanation (\emph{i.e.}, multi-tasks learning); \textbf{v) \cite{chang2021towards}} that augmented the dataset with various factual and counterfactual images to alleviate the problem of learning spurious features; and \textbf{vi)} the \textbf{Oracle classifier} in which we manually restrict the input features to areas annotated by radiologists.

\begin{table}[htp]
  \caption{Comparison with baseline methods on LIDC-IDRI and CBIS-DDSM datasets. The result of our method is \textbf{boldfaced} and the best result among baseline methods is \underline{underlined}. For the Oracle classifier, the input features are manually restricted to the areas annotated by radiologists.}
  \label{tab.cmp-baselines}
  \centering
  \begin{tabular}{lllll}
    \toprule
    \multirow{2}{*}{Methodology} \qquad\qquad  & \multicolumn{2}{l}{Precision of CAM \quad\quad}  & \multicolumn{2}{l}{Classification accuracy} \\
    \cmidrule(r){2-5}
         & LIDC & DDSM  & LIDC & DDSM \\
    
    \midrule
    \cite{ross2017right} & 0.034 (0.06) & 0.084 (0.11) & \underline{0.656 (0.00)} & 0.559 (0.05) \\
    \cite{zhang2018interpretable} &  0.068 (0.11) & 0.110 (0.13) & 0.381 (0.03) & 0.581 (0.00) \\
    \cite{brendel2019approximating} & 0.048 (0.04) &0.090 (0.04) & 0.358 (0.00) & \underline{0.592 (0.00)} \\
    \cite{rieger2020interpretations} & 0.041 (0.05) & \underline{0.232 (0.17)} & 0.343 (0.00) & 0.586 (0.01)  \\
    \cite{chang2021towards} & \underline{0.074 (0.03)}  & 0.119 (0.07) & 0.503 (0.08) & 0.496 (0.08)  \\
    Oracle classifier & 1.000 (0.00) & 1.000 (0.00) & 0.789 (0.00) & 0.726 (0.01) \\
    \midrule
    Ours & \textbf{0.751 (0.03)}  &\textbf{0.805 (0.06)}   & \textbf{0.722 (0.00)} & \textbf{0.656 (0.00)}   \\
    \bottomrule
  \end{tabular}
\end{table}

\textbf{Results \& Analysis.} Tab.~\ref{tab.cmp-baselines} reports the alignment precision and classification accuracy. As shown, our method demonstrates strong alignment with radiologists in the diagnostic process. This result verifies the utility of our alignment loss and the optimization process. In contrast, other methods with no alignment may learn unreliable features that are beyond the annotated areas, which deteriorates their prediction accuracy. Specifically, one should note that ICNN \cite{zhang2018interpretable}, BagNet \cite{brendel2019approximating}, and \cite{rieger2020interpretations} imposed no explicit constraint for learning explainable features. As a result, these methods can be easily biased by background features or pseudo-correlations in the image. Meanwhile, although methods such as \cite{ross2017right} and \cite{chang2021towards} explicitly constrained the input gradient to human decision areas, the gradient method itself has been criticized for being unable to represent full model decision boundary \cite{jain2019attention,grimsley2020attention}, making their constraints less effective. 

Due to its capability to capture causal features, our method also significantly surpasses baseline models in terms of classification accuracy. This can be attributed to the fact that, unlike the ``$+$"/``$-$" symbol, which demonstrates only spurious correlation to the label, features within the annotated areas have a causal relationship with the label, and therefore are transferable to test data.

Additionally, it is worth noting from Tab.~\ref{tab.cmp-baselines} that even the oracle classifier only reaches an classification accuracy of $65\%$ - $72\%$, which seems to contradict some previous results \cite{wu2018joint,wang2022disentangling} that claimed an accuracy of more than $99\%$ in lung nodule classification and $90\%$ in breast mass classification. To comprehend, this discrepancy is primarily due to the exclusion of challenging samples (those with a malignancy score of $3$) in \cite{wu2018joint}, and the usage of custom training/test sets split in \cite{wang2022disentangling}. 



\subsection{Ablation Study}

In this section, we perform an ablation study on the causal alignment loss (Sec.\ref{sect.loss}) and the hierarchical optimization process (Sec.\ref{sect.hierachy}). The results are shown in Tab.~\ref{tab.ablation-study}. 

\begin{table}[htp]
  \caption{Ablation study on LIDC-IDRI and CBIS-DDSM datasets.}
  \label{tab.ablation-study}
  \centering
  \begin{tabular}{ccllll}
    \toprule
    \multirow{2}{*}{$\mathcal{L}_{\text{align}}$} & \multirow{2}{*}{Hierarchical align\,\,\,}  & \multicolumn{2}{l}{Precision of CAM \quad\quad}  & \multicolumn{2}{l}{Classification accuracy} \\
    \cmidrule(r){3-6}
       &  & LIDC & DDSM  & LIDC & DDSM \\
    
    \midrule
    $\times$ & $\times$ & 0.057 (0.07) & 0.143 (0.20) & 0.535 (0.08)& 0.592 (0.00)   \\
    \checkmark & $\times$ & 0.587 (0.08) & 0.621 (0.03) & 0.701 (0.02) & 0.633 (0.03) \\
    \checkmark & \checkmark & \textbf{0.751 (0.03)} & \textbf{0.805 (0.06)} & \textbf{0.722 (0.00)} & \textbf{0.656 (0.00)}    \\
    \bottomrule
  \end{tabular}
\end{table}

As we can see, both the alignment loss and the hierarchical optimization enhance the performance of our method. In detail, the alignment loss accounts for a substantial portion of the improvement, yielding a $50\%$ increase in CAM precision and a $15\%$ boost in classification accuracy. Additionally, the hierarchical training strategy contributes an extra $20\%$ to alignment precision and a $2\%$ increase in classification performance. These results demonstrate the effectiveness of our alignment loss in learning features that coincide with radiologist assessments, as well as the significance of the hierarchical training strategy in mimicking the clinical diagnosis process.


\subsection{Visualization}

To further verify whether our method can learn radiologist-aligned features, we visualize the Class Activation Mapping (CAM) and show the results in Fig.~\ref{fig.visu-grad-cam}. The first two rows of Fig.~\ref{fig.visu-grad-cam} present cases with lung nodules while the third and the fourth rows present cases with breast masses. The first column shows the input image, with the nodule/mass areas marked by red bounding boxes, while other columns present CAMs of various models. 

\begin{figure}[htp]
    \centering
    \includegraphics[width=\textwidth]{fig/visu_cmp_baselines.pdf}
    \caption{CAM visualization. Each row denotes different cases. The first column is the input images, where nodules and masses are marked by red bounding boxes. The second to seventh columns are CAMs of compared baselines and our method, respectively. Please refer to Appx.~\ref{appx.more-visu} for more results.}
    \label{fig.visu-grad-cam}
\end{figure}

As we can see, the activation of our method concentrates on the nodule/mass areas, especially on the margins of the nodules/mass, which is a key feature for radiologists to evaluate the malignancy \cite{sandler2023acr}. In contrast, the activation of baseline methods focuses on lesion-irrelevant areas, such as the shortcut symbol ``$+$"/``$-$" region in the top-left corner for \cite{ross2017right} and BagNet \cite{brendel2019approximating}, or the background areas like the pleural and spine for ICNN \cite{zhang2018interpretable}, \cite{rieger2020interpretations}, and \cite{chang2021towards}. This visual analysis corroborates the quantitative results, demonstrating our method's ability to learn features that are well-aligned with the radiologists' diagnostic process.


==> para/introduction.tex <==
\section{Introduction}

Alignment is essential for developing reliable medical diagnosis systems \cite{zhuang2020consequences,raji2022fallacy}. For instance, in lung cancer diagnosis, using models that are misaligned with clinical protocols can result in reliance on contextual features or instrument markers (Fig.~\ref{fig.intro} (c)) for prediction, leading to misdiagnosis and loss of timely treatment.

Despite the importance, alignment in medical imaging systems is largely understudied. Other works that are mostly related to us include \cite{zhang2018interpretable,chen2019looks,brady2023provably} that proposed to learn object-centric representations, and \cite{hind2019ted,rieger2020interpretations} that adopted multi-task learning schemes to predict labels and expert decision bases simultaneously. Particularly, recent works \cite{ross2017right,gao2022aligning,zhang2023magi} have proposed to regularize the model's input gradient to be within expert-annotated areas. However, their alignment with expert behaviors is only associational, rather than causal, making their models still biased towards spurious correlated features. This drawback is further explained in Fig.~\ref{fig.intro} (a), where two decision chains with different causal structures can exhibit similar correlation patterns.

\begin{figure}[t!]
    \centering
    \includegraphics[width=1.0\textwidth]{fig/intro.pdf}
    \caption{(a) Two decision chains with different causal structures but present similar correlation patterns. The left chain ``$\text{mass } (X) \!\to\! \text{attributes } (A) \!\to\! \text{label } (Y)$'' aligns with radiologists, while the right chain ``$\text{shortcut} \!\to\! \text{label } (Y)$'' is misaligned. However, the two chains have similar correlation patterns due to the confounding between the mass and shortcut mark. (b) Our approach for learning causally aligned model. We first identify features and attributes that causally influence the model's decision, then align them to that of radiologists in a hierarchical fashion. (c) Class Activation Mapping (CAM) visualization and comparison of CAM precision on lung cancer diagnosis.}
    \label{fig.intro}
\end{figure}

In this paper, we propose a causality-based framework to align the underlying causal mechanism of the decision-making process. Taking the clinical decision chain as a reference, we first identify features that have causal influence on the model's decision using counterfactual generation. We then propose a causal alignment loss to enforce these identified causal areas to be aligned within those annotated by the radiologists. To optimize this loss that involves an implicit function of the model parameters, we employ the implicit function theorem equipped with the conjugate gradient algorithm for efficient estimation. Finally, we incorporate our alignment loss to train a hierarchical prediction model (Fig.~\ref{fig.intro} (b)) that mimics the clinical decision pipeline, which first describes attributes of the lesion, and then diagnoses based on these attributes. Such training is facilitated by employing causal attribution \cite{zhao2023conditional} for inferring attributes that are causally related to the diagnosis. Returning to the lung cancer diagnosis example, Fig.~\ref{fig.intro} (c) shows that our method can learn causally aligned representations, in contrast to the features adopted by baseline methods, which are challenging to interpret.

\vspace{+1cm}
\textbf{Contributions.} To summarize, our contributions are:
\begin{enumerate}
    \item We propose a novel causal alignment loss to align the model's decision chain with that of experienced radiologists. 
    \item We propose using the implicit function theorem for efficient optimization.
    \item We achieve more accurate alignment and prediction than existing methods on lung cancer and breast cancer diagnosis.
\end{enumerate}


==> para/method.tex <==
\section{Methodology}

\begin{figure}[tp]
    \centering
    \includegraphics[width=1.0\textwidth]{neurips24/fig/framework.pdf}
    \caption{The schematic overview of our method. (a) We adopt a hierarchical structure that first provides attribute descriptions for the image, and then shows the diagnosis result. (b) Training with the proposed alignment loss. In the forward pass, a counterfactual image $x^*$ is generated and used to compute the alignment loss $\mathcal{L}_{\text{align}}$ relative to the expert's annotation $s$. In the backward pass, we use an implicit gradient solver to obtain the gradient $\nabla_\theta \mathcal{L}_{\text{align}}$ and use it to update the parameter $\theta$.}
    \label{fig.overview}
\end{figure}

In this section, we introduce our framework for medical decision alignment. This section is composed of three parts. First, in Sect.~\ref{sect.loss}, we introduce a \emph{causal alignment loss} based on counterfactual generation, to align the model's decision basis with those of experts. Then, in Sect.~\ref{sect.optim}, we propose to use the Implicit Function Theorem (IFT) equipped with conjugate gradient estimation to compute the gradient of our loss for optimization. Finally, in Sect.~\ref{sect.hierachy}, we enhance our method with hierarchical alignment for cases where attribute annotations are available, using a hierarchical optimization pipeline based on causal attribution. We summarize our framework in Fig.~\ref{fig.overview}.

\subsection{Casual Alignment Loss}
\label{sect.loss}

In this section, we proposal a causal alignment loss to align the model with experts. For illustration, we first consider the case where the attribute annotations are unavailable.

The idea of our loss is to penalize the model once its counterfactual image has modifications beyond the areas annotated by radiologists. Specifically, we let the annotation matrix $s\in \{0,1\}^{\mathrm{dim}(x)}$, which is a binary mask indicating whether the feature $j\in \{1,...,\mathrm{dim}(x)\}$ should be responsible for the prediction of the label $y$. Then, we would like the counterfactual modification $\left|x^* - x\right|$ to be small at locations that are not responsible for the prediction. To this end, we optimize a loss $\mathcal{L}_{\text{align}}$ of the following form:
\begin{equation}
    \mathcal{L}_{\text{align}} := \frac{1}{n} \sum_{i=1}^n \left\|(x^*_i- x_i) \odot (1-s_i)\right\|_{1},
    \label{eq.our loss}
\end{equation}
where $\odot$ denotes the element-wise Hadamard matrix product and $x^*_i(\theta)$ is the counterfactual image of $x_i$ obtained from Eq.~\ref{eq.objective.cf}. In other words, the alignment loss is an $\ell_1$-norm that penalizes the counterfactual image to modify within the expert's annotations. 

Then, by combining Eq.~\ref{eq.our loss} with the cross-entropy loss for classification, we can obtain our overall training objective:
\begin{equation*}
    \mathcal{L} = \mathcal{L}_{\text{ce}} + \lambda \mathcal{L}_{\text{align}}, 
\end{equation*}
where $\lambda$ is a tuning hyperparameter.

To understand how the objective works towards alignment, note that the $\ell_1$-norm in Eq.~\ref{eq.our loss} penalizes the model if the counterfactual image has modifications beyond expert-annotated regions, which can lead to an insensitivity of $f_\theta$ to features beyond expert's view. In this regard, to achieve a low classification loss, the model will be forced to learn features within expert-annotated regions, thereby achieving the desired alignment. 

Our loss enjoys several advantages over alternative methods in visual alignment. Compared to \cite{zhang2018interpretable,liu2021act,wang2022knowledge} that incorporated prior knowledge into the network architecture for explainability, our loss is more flexible and can be easily adapted to other scenarios and backbones. In contrast to \cite{ross2017right,ismail2021improving,gao2022aligning} that constrained the input gradient, our approach can achieve more accurate alignment and avoid potential pseudo-features, benefiting from the identification of causal features. 

\subsection{Optimization}
\label{sect.optim}

In this section, we introduce the optimization process for the proposed alignment loss. To optimize Eq.~\ref{eq.our loss}, we need to compute the gradient $\nabla_\theta \mathcal{L}_{\text{align}}$, which involves the Jacobian matrix $\nabla_\theta x^*$. The main challenge here is that $x^*$ is an \emph{implicit function} of $\theta$, defined by the argmin operator in Eq.~\ref{eq.objective.cf}, which makes it hard to compute $\nabla_\theta x^*$ explicitly. 

To address this challenge, we resort to the Implicit Function Theorem (IFT), which allows us to compute the gradient in an implicit manner. Specifically, note that if $x^*$ is the minimum point of the function $T(x,\theta) := \mathcal{L}_{\text{ce}}(f_\theta(x),y^*) + \alpha d(x,x_0)$, it should satisfy that:
\begin{equation*}
    \nabla_x T \Bigr|_{x^*} = 0.
\end{equation*}

According to the law of total derivation, this implies that:
\begin{equation*}
    \nabla_\theta \nabla_x T \Bigr|_{x^*} = \{\nabla_x (\nabla_x T) \cdot \, \nabla_\theta x^* + \nabla_\theta (\nabla_x T)\} \Bigr|_{x^*} = 0.
\end{equation*}

Therefore, computing $\nabla_\theta x^*$ boils down to the problem of solving the following linear equations:
\begin{equation}
    H z^* = b,
    \label{eq.linear-eq}
\end{equation}
where we denote $H:=\nabla_x (\nabla_x T)$ as the Hessian matrix, $z^* :=\nabla_\theta x^*$ as the Jacobian matrix, and $b:=-\nabla_\theta (\nabla_x T)$ as the negative mixed derivative for brevity. 

Formally speaking, we have the following theorem:
\begin{theorem}[Implicit Function Theorem (IFT) \cite{krantz2002implicit}]
    Consider two vectors $x, \theta$, and a differentiable function $T(x,\theta)$. Let $x^* := \arg\min_x T(x,\theta)$. Suppose that: \textbf{i)} the argmin is unique for each $\theta$, and \textbf{ii)} the Hessian matrix $H$ is invertible. Then $x^*(\theta)$ is a continuous function of $\theta$. Further, the Jacobian matrix $\nabla_\theta x^*$ satisfies the linear Eq.~\ref{eq.linear-eq}.
    \label{thm.ift}
\end{theorem}

Thm.~\ref{thm.ift} suggests that we can compute the Jacobian matrix using $\nabla_\theta x^* = - H^{-1} b$, which then gives $\nabla_\theta \mathcal{L}_{\text{align}}$ with the chain-rule. Nonetheless, for imaging tasks, typically $\theta$ is the parameter of high-dimensional neural networks, making it intractable to compute the Hessian matrix and its inverse. To address this issue, we employ the conjugate gradient algorithm \cite{vishnoi2013lx} to estimate the solution of Eq.~\ref{eq.linear-eq}, without explicitly computing or storing the Hessian matrix. Notably, the conjugate gradient method has been successfully deployed in Hessian-free methods for deep learning \cite{nesterov2006cubic,martens2010deep} and meta learning \cite{rajeswaran2019meta,sitzmann2020metasdf}.

We briefly introduce the idea of conjugate gradient method below, with a detailed discussion left to \cite{vishnoi2013lx} (Chap.~6). To begin with, note that solving Eq.~\ref{eq.linear-eq} is equivalent to solving
\begin{equation*}
    z^* = \arg\min_{z} g(z), \,\, \text{where} \,\, g(z):=\frac{1}{2} {z}^\top H z - b^\top z,
\end{equation*}
in that the minimum point $z^*$ satisfies $\nabla_{z} g \Bigr|_{z^*} = Hz^* - b = 0$. 

In this regard, we can implement gradient descent to minimize $g(\cdot)$, where the minimum point gives the solution of Eq.~\ref{eq.linear-eq}. During the minimization, the direction of the gradient updating is set to be conjugate (\emph{i.e.}, orthogonal) to the residual $b-H z^{(i)}$, where $z^{(i)}$ is the estimate of $z^*$ in the $i$-th iteration, in order to achieve optimal convergence rate. 

To achieve this without explicitly forming $H$, we can leverage the \emph{Hessian vector product} \cite{song2022modeling}. Specifically, for $\epsilon$ that is a small perturbation around $z$, we have:
\begin{equation*}
    \nabla g(z+ \epsilon z^{(i)}) \approx \nabla g(z) + H \epsilon z^{(i)}.
\end{equation*}
It then follows that:
\begin{equation*}
    H z^{(i)} \approx \frac{\nabla g(z+ \epsilon z^{(i)}) - \nabla g(z)}{\epsilon},
\end{equation*}
which means we can estimate $H z^{(i)}$ with the finite difference of $\nabla g$ on the right-hand side.

Equipped with Thm.~\ref{thm.ift} especially the conjugate gradient method for estimation, we now summarize the optimization process for our alignment loss in Alg.~\ref{alg:optimization}.

\algnewcommand\algorithmichyper{\textbf{Hyperparameters:}}
\algnewcommand\Hyperparameter{\item[\algorithmichyper]}

\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}

\begin{algorithm}[htp]
\caption{Optimization for $\mathcal{L}_{\text{align}}$}
\label{alg:optimization}
\begin{algorithmic}[1]
\Input Data $\mathcal{D}$, model $f_\theta$, 
\Hyperparameter{Sparsity regularization $\alpha$, learning rate $\eta$}
\While{not converged}
\State Optimize Eq.~\ref{eq.objective.cf} to obtain $x^*$.
\State Compute $\mathcal{L}_{\text{align}}$ using Eq.~\ref{eq.our loss}.
\State Estimate $\nabla_\theta \mathcal{L}_{\text{align}}$ with conjugate gradient. 
\State Update $\theta$ with gradient descent: $\theta \leftarrow \theta-\eta \nabla_\theta \mathcal{L}_{\text{align}}$.  \,\, \text{// \emph{or Adam}}
\EndWhile
\end{algorithmic}
\end{algorithm}



\subsection{Hierarchical Alignment}
\label{sect.hierachy}

In this section, we consider the scenario where the attribute annotations are available. We introduce a hierarchical alignment framework to mirror the clinical diagnostic procedure, where radiologists typically start by analyzing a patient's symptoms and then diagnose the disease based on these symptom analyses \cite{xie2020chexplain}.

Specifically, our classifier $f_\theta$ consists of an $f_{\theta_1}:\mathcal{X}\mapsto\mathcal{A}$ that predicts the attributes from the input image $x$, and an $f_{\theta_2}:\mathcal{A} \mapsto \mathcal{Y}$ that classifies the label based on the predicted attributes. \emph{During the backward optimization}, we first find attributes responsible for the prediction of $y$ by altering the original attributes $a$ to the counterfactual class $a^*$. Then, we locate image features that accounts for the modification of $|a^*-a|$ via another counterfactual optimization over $x$ and obtaining the counterfactual image $x^*$. For hierarchical alignment, we require both $|a^*-a|$ and $|x^*-x|$ to be aligned with the expert's annotations of causal attributes and image regions, respectively. 

\textbf{Causal Attribution for Annotations.} Although the attribute annotation can be available for many cases \cite{armato2011lung,lee2017curated}, it is hard to know which ones of these attributes are causally related to the disease label. To infer the causal attributes for optimization, we employ causal attribution based on counterfactual causal effect \cite{zhao2023conditional}. Specifically, given evidence of the attributes $A=a$ and the label $Y=y$, we calculate the Conditional Counterfactual Causal Effect (CCCE) score for each attribute subset $S\subseteq \{1,...,\mathrm{dim}(A)\}$
\begin{equation*}
    \text{CCCE}(S):=\mathbb{E}(Y_{A_S=1} - Y_{A_S=0} | A=a, Y = y),
\end{equation*}
which is the difference between the conditional expectations of the potential outcomes $Y_{A_S=1}$ and $Y_{A_S=0}$ given the evidence. 

According to \cite{zhao2023conditional} (Thm.~2), this quantity is identifiable and equals to
\begin{equation*}
    1 - \frac{\mathrm{P}\left(Y_{A_S=1}=y \mid A=a\right)}{\mathrm{P}(Y=y \mid A=a)}
\end{equation*}
under the monotonicity condition that $Y_{a} \leq Y_{a^\prime}$ if $a\preceq a^\prime$ \footnote{Here, $a$ and $a^\prime$ are both vectors. $a \preceq a^\prime$ denotes $a_k \leq a^\prime_k$ for each $k$.}. This condition is natural to hold in our scenario, since for each intervention on any attribute from $0$ to $1$ (\emph{e.g.}, from no speculation to speculation) will raise the probability of malignancy. 

After computing the CCCE score for each attribute subset, we then select the subset $S$ with the highest CCCE as the set of attributes that are causally related to the label. Accordingly, we set the annotation vector $r \in \{0,1\}^{\mathrm{dim}(A)}$ such that $r_S=(1,...,1)^\top$. 

\textbf{Hierarchical Optimization.} With such annotations, we propose a hierarchical optimization process. To be specific, we first generate the counterfactual attributes $a^*$ using
\begin{equation}
    a^* = \arg\min_{a^\prime} \mathcal{L}_{\text{ce}}(f_{\theta_2}(a^\prime),y^*) + \alpha_2 {d}(a^\prime,a),
\label{eq.counter-attribute}
\end{equation}
where $y^*:=1- y$ is the counterfactual label and $a$ denotes the original attributes.

We then optimize $\theta_2$ with
\begin{equation*}
    \mathcal{L}(\theta_2):=\mathcal{L}_{\text{ce}}(\theta_2) + \lambda_2 \mathcal{L}_{\text{align}}(\theta_2), 
\end{equation*}
where the alignment loss over $\theta_2$ is defined as
\begin{equation*}
    \mathcal{L}_{\text{align}}(\theta_2) := \frac{1}{n} \sum_{i=1}^n \left\|(a^*_i - a_i) \odot (1-r_i)\right\|_{\ell_1}.
    \label{eq.our loss 1}
\end{equation*}
Then, in the second stage, we perturb the original image $x$ to obtain the counterfactual image $x^*$ that explains the change of $a$ to $a^*$
\begin{equation*}
    x^* = \arg\min_{x^\prime} \mathcal{L}_{\text{ce}}(f_{\theta_1}(x^\prime),a^*) + \alpha_1 {d}(x^\prime,x).  
\label{eq.counter-image-2}
\end{equation*}
We then optimize $\theta_1$ with
\begin{equation*}
    \mathcal{L}(\theta_1):=\mathcal{L}_{\text{ce}}(\theta_1) + \lambda_1 \mathcal{L}_{\text{align}}(\theta_1), 
\end{equation*}
where the alignment loss over $\theta_1$ is given by Eq.~\ref{eq.our loss}. 


==> para/method_xw_v1.tex <==
\section{Methodology}

\begin{figure}[tp]
    \centering
    \includegraphics[width=1.0\textwidth]{neurips24/fig/framework.pdf}
    \caption{The schematic overview of our method. (a) We adopt a hierarchical structure that first provides attribute descriptions for the image, and then shows the diagnosis result. (b) Training with the proposed alignment loss. In the forward pass, a counterfactual image $x^*$ is generated and used to compute the alignment loss $\mathcal{L}_{\text{align}}$ relative to the expert's annotation $s$. In the backward pass, we use an implicit gradient solver to obtain the gradient $\nabla_\theta \mathcal{L}_{\text{align}}$ and use it to update the parameter $\theta$.}
    \label{fig.overview}
\end{figure}

In this section, we introduce our framework for medical decision alignment. This section is composed of three parts. First, in Sect.~\ref{sect.loss}, we introduce a \emph{causal alignment loss} based on counterfactual generation, to align the model's decision basis with those of experts. Then, in Sect.~\ref{sect.optim}, we propose to use the Implicit Function Theorem (IFT) equipped with conjugate gradient estimation to compute the gradient of our loss for optimization. Finally, in Sect.~\ref{sect.hierachy}, we enhance our method with hierarchical alignment for cases where attribute annotations are available, using a hierarchical optimization pipeline based on causal attribution. We summarize our framework in Fig.~\ref{fig.overview}.

\subsection{Casual Alignment Loss}
\label{sect.loss}

In this section, we proposal a causal alignment loss to align the model with the experts. For illustration, we first consider the case where the attribute annotations are unavailable.

The idea of our loss is to penalize the model once its counterfactual image contains modifications beyond radiologist-annotated areas. Specifically, we let the annotation matrix $s\in \{0,1\}^{\mathrm{dim}(x)}$ be a binary mask indicating whether the feature $j\in \{1,...,\mathrm{dim}(x)\}$ should be responsible for the prediction of the label $y$. Then, we would like the counterfactual modification $\left|x^* - x\right|$ to be small at locations that are not responsible for the prediction. To this end, we optimize a loss $\mathcal{L}_{\text{align}}$ of the following form:
\begin{equation}
    \mathcal{L}_{\text{align}} := \frac{1}{n} \sum_{i=1}^n \left\|(x^*_i- x_i) \odot (1-s_i)\right\|_{1},
    \label{eq.our loss}
\end{equation}
where $\odot$ denotes the element-wise Hadamard matrix product and $x^*_i$ is the counterfactual image of $x_i$ obtained from Eq.~\ref{eq.objective.cf}.

Then, by combining Eq.~\ref{eq.our loss} with the cross-entropy loss for classification, we can obtain our overall training objective:
\begin{equation*}
    \mathcal{L} = \mathcal{L}_{\text{ce}} + \lambda \mathcal{L}_{\text{align}}, 
\end{equation*}
where $\lambda$ is a tuning hyperparameter.

To understand how the objective works towards alignment, note that the $\ell_1$-norm in Eq.~\ref{eq.our loss} penalizes the model if the counterfactual image has modifications beyond expert-annotated regions, which can lead to an insensitivity of $f_\theta$ to features beyond expert's view. In this regard, the model will be forced to learn features within expert-annotated regions for prediction, thereby achieving the desired alignment\footnote{This is formalized in Claim~\ref{claim.causal-alignment} in the appendix.}. 


Our loss enjoys several advantages over alternative methods in visual alignment. Compared to \cite{zhang2018interpretable,liu2021act,wang2022knowledge} that incorporated prior knowledge into the network architecture for explainability, our loss is more flexible and can be easily adapted to other scenarios and backbones. In contrast to \cite{ross2017right,ismail2021improving,gao2022aligning} that constrained the input gradient, our approach can achieve more accurate alignment and avoid potential pseudo-features, benefiting from the identification of causal features. 

\subsection{Optimization}
\label{sect.optim}

In this section, we introduce the optimization process for the proposed alignment loss. To optimize Eq.~\ref{eq.our loss}, we need to compute the gradient $\nabla_\theta \mathcal{L}_{\text{align}}$, which involves the Jacobian matrix $\nabla_\theta x^*$. The main challenge here is that $x^*$ is an \emph{implicit function} of $\theta$, defined by the argmin operator in Eq.~\ref{eq.objective.cf}, which makes it hard to compute $\nabla_\theta x^*$ explicitly. 

To address this challenge, we resort to the Implicit Function Theorem (IFT), which allows us to compute the gradient in an implicit manner. Specifically, note that if $x^*$ is the minimum point of the function $T(x,\theta) := \mathcal{L}_{\text{ce}}(f_\theta(x),y^*) + \alpha d(x,x_0)$, it should satisfy that:
\begin{equation*}
    \nabla_x T \Bigr|_{x^*} = 0.
\end{equation*}

According to the law of total derivation, this implies that:
\begin{equation*}
    \nabla_\theta \nabla_x T \Bigr|_{x^*} = \{\nabla_x (\nabla_x T) \cdot \, \nabla_\theta x^* + \nabla_\theta (\nabla_x T)\} \Bigr|_{x^*} = 0.
\end{equation*}

Therefore, computing $\nabla_\theta x^*$ boils down to the problem of solving the following linear equations:
\begin{equation}
    H z^* = b,
    \label{eq.linear-eq}
\end{equation}
where we denote $H:=\nabla_x (\nabla_x T)$ as the Hessian matrix, $z^* :=\nabla_\theta x^*$ as the Jacobian matrix, and $b:=-\nabla_\theta (\nabla_x T)$ as the negative mixed derivative for brevity. 

Formally speaking, we have the following theorem:
\begin{theorem}[Implicit Function Theorem (IFT) \cite{krantz2002implicit}]
    Consider two vectors $x, \theta$, and a differentiable function $T(x,\theta)$. Let $x^* := \arg\min_x T(x,\theta)$. Suppose that: \textbf{i)} the argmin is unique for each $\theta$, and \textbf{ii)} the Hessian matrix $H$ is invertible. Then $x^*(\theta)$ is a continuous function of $\theta$. Further, the Jacobian matrix $\nabla_\theta x^*$ satisfies the linear Eq.~\ref{eq.linear-eq}.
    \label{thm.ift}
\end{theorem}

Thm.~\ref{thm.ift} suggests that we can compute the Jacobian matrix using $\nabla_\theta x^* = - H^{-1} b$, which then gives $\nabla_\theta \mathcal{L}_{\text{align}}$ with the chain-rule. Nonetheless, for imaging tasks, typically $\theta$ is the parameter of high-dimensional neural networks, making it intractable to compute the Hessian matrix and its inverse. To address this issue, we employ the conjugate gradient algorithm \cite{vishnoi2013lx} to estimate the solution of Eq.~\ref{eq.linear-eq}, without explicitly computing or storing the Hessian matrix. Notably, the conjugate gradient method has been successfully deployed in Hessian-free methods for deep learning \cite{nesterov2006cubic,martens2010deep} and meta learning \cite{rajeswaran2019meta,sitzmann2020metasdf}.

We briefly introduce the idea of conjugate gradient method below, with a detailed discussion left to \cite{vishnoi2013lx} (Chap.~6). To begin with, note that solving Eq.~\ref{eq.linear-eq} is equivalent to solving
\begin{equation*}
    z^* = \arg\min_{z} g(z), \,\, \text{where} \,\, g(z):=\frac{1}{2} {z}^\top H z - b^\top z,
\end{equation*}
in that the minimum point $z^*$ satisfies $\nabla_{z} g \Bigr|_{z^*} = Hz^* - b = 0$. 

In this regard, we can implement gradient descent to minimize $g(\cdot)$, where the minimum point gives the solution of Eq.~\ref{eq.linear-eq}. During the minimization, the direction of the gradient updating is set to be conjugate (\emph{i.e.}, orthogonal) to the residual $b-H z^{(i)}$, where $z^{(i)}$ is the estimate of $z^*$ in the $i$-th iteration, in order to achieve optimal convergence rate. 

To achieve this without explicitly forming $H$, we can leverage the \emph{Hessian vector product} \cite{song2022modeling}. Specifically, for $\epsilon$ that is a small perturbation around $z$, we have:
\begin{equation*}
    \nabla g(z+ \epsilon z^{(i)}) \approx \nabla g(z) + H \epsilon z^{(i)}.
\end{equation*}
It then follows that:
\begin{equation*}
    H z^{(i)} \approx \frac{\nabla g(z+ \epsilon z^{(i)}) - \nabla g(z)}{\epsilon},
\end{equation*}
which means we can estimate $H z^{(i)}$ with the finite difference of $\nabla g$ on the right-hand side.

Equipped with Thm.~\ref{thm.ift} especially the conjugate gradient method for estimation, we now summarize the optimization process for our alignment loss in Alg.~\ref{alg:optimization}.

\algnewcommand\algorithmichyper{\textbf{Hyperparameters:}}
\algnewcommand\Hyperparameter{\item[\algorithmichyper]}

\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}

\begin{algorithm}[htp]
\caption{Optimization for $\mathcal{L}_{\text{align}}$}
\label{alg:optimization}
\begin{algorithmic}[1]
\Input Data $\mathcal{D}$, model $f_\theta$, 
\Hyperparameter{Sparsity regularization $\alpha$, learning rate $\eta$}
\While{not converged}
\State Optimize Eq.~\ref{eq.objective.cf} to obtain $x^*$.
\State Compute $\mathcal{L}_{\text{align}}$ using Eq.~\ref{eq.our loss}.
\State Estimate $\nabla_\theta \mathcal{L}_{\text{align}}$ with conjugate gradient. 
\State Update $\theta$ with gradient descent: $\theta \leftarrow \theta-\eta \nabla_\theta \mathcal{L}_{\text{align}}$.  \,\, \text{// \emph{or Adam}}
\EndWhile
\end{algorithmic}
\end{algorithm}



\subsection{Hierarchical Alignment}
\label{sect.hierachy}

In this section, we extend our method to the scenario where attribute annotations are available. We introduce a hierarchical alignment framework to mimic the clinical diagnostic procedure, where radiologists typically start by analyzing a patient's symptoms and then diagnose the disease based on these symptom analyses \cite{xie2020chexplain}.

Specifically, our classifier $f_\theta$ consists of an $f_{\theta_1}:\mathcal{X}\mapsto\mathcal{A}$ that predicts the attributes from the input image $x$, and an $f_{\theta_2}:\mathcal{A} \mapsto \mathcal{Y}$ that classifies the label based on the predicted attributes, where $\theta_1$ and $\theta_2$ are optimized in an end-to-end manner. \emph{During the counterfactual generation}, we first find attributes $a^*(\theta_2)$ responsible for the prediction of $y$ by altering the predicted attributes $\wh{a}:=f_{\theta_1}(x)$ to the counterfactual class $y^*$. Then, we locate image features that accounts for the modification of $|a^*(\theta_2)-\wh{a}|$ via another counterfactual optimization over $x$ and obtaining the counterfactual image $x^*$. For hierarchical alignment, we require both $|a^*(\theta_2)-\wh{a}|$ and $|x^*(\theta_1)-x|$ to be aligned with the expert's annotations of causal attributes and image regions, respectively. 

\textbf{Causal Attribution for Annotations.} Although the attribute annotation can be available for many cases \cite{armato2011lung,lee2017curated}, it is hard to know which ones of these attributes are causally related to the disease label. To identify the causal attributes for alignment, we employ causal attribution based on counterfactual causal effect \cite{zhao2023conditional}, which extends Eq.~\ref{eq.coe} to enable the quantification of the probability of causation for any subsets of attributes while conditioning on the entire attribute vector. Specifically, given evidence of the attributes $A=a$ and the label $Y=y$, we calculate the Conditional Counterfactual Causal Effect (CCCE) score for each attribute subset $S\subseteq \{1,...,\mathrm{dim}(A)\}$
\begin{equation*}
    \text{CCCE}(S):=\mathbb{E}(Y_{A_S=1} - Y_{A_S=0} | A=a, Y = y),
\end{equation*}
which is the difference between the conditional expectations of the potential outcomes $Y_{A_S=1}$ and $Y_{A_S=0}$ given the evidence. 

Recall that each attribute $A_i$ is binary. Then, according to \cite{zhao2023conditional} (Thm.~2), $\text{CCCE}(S)$ is identifiable and equals to
\begin{equation*}
    \text{CCCE}(S) \overset{(1)}{=} 1 - \frac{\mathrm{P}\left(Y_{A_S=\bm{1}_S}=y \mid A=a\right)}{\mathrm{P}(Y=y \mid A=a)} \overset{(2)}{=} 1 - \frac{\mathrm{P}\left(Y=y \mid A_S = \bm{1}_S, A_{-S} = a_{-S}\right)}{\mathrm{P}(Y=y \mid A=a)},
\end{equation*}
where ``(1)" arises from the exogeneity condition that there is no counfounding between $A$ and $Y$ (\emph{i.e.}, $Y_a \perp A$), and ``(2)" is based on the monotonicity condition \footnote{\cite{zhao2023conditional} also assumed exogeneity condition and the monotonicity conditions among $A$, if there exists causal relations among $A$. Since there are no causal relations among $A$, we do not need these conditions.} that $Y_{a} \leq Y_{a^\prime}$ if $a\preceq a^\prime$ \footnote{Here, $a$ and $a^\prime$ are both vectors. $a \preceq a^\prime$ denotes $a_k \leq a^\prime_k$ for each $k$.}. Both conditions are natural to hold in our scenario. Specifically, the exogeneity condition holds since radiologists' decision $Y$ are based only on attributes. For the monotonicity condition, it is easy to see that for each intervention on any attribute from $0$ to $1$ (\emph{e.g.}, from no speculation to speculation) will raise the probability of malignancy. 

%This condition is natural to hold in our scenario, since for each intervention on any attribute from $0$ to $1$ (\emph{e.g.}, from no speculation to speculation) will raise the probability of malignancy. 

After computing the CCCE score for each attribute subset, we then select the subset $S$ with the highest CCCE as the set of attributes that are causally related to the label. Accordingly, we set the annotation vector $r \in \{0,1\}^{\mathrm{dim}(A)}$ such that $r_S=(1,...,1)^\top$. 

\textbf{Alignment.} With such annotations, we introduce our alignment process. Specifically, our objective function over $(\theta_1,\theta_2)$ is:
\begin{equation}
    \label{eq.objective}
    \cL_{\lambda_1,\lambda_2,\lambda_3}(\theta_1,\theta_2) := \cL_{\text{ce}}(f_{\theta_2}(f_{\theta_1}(x)),y) + \lambda_1 \cL_{\text{ce}}(f_{\theta_1}(x), a) + \lambda_2 \mathcal{L}_{\text{align}}(\theta_2) + \lambda_3 \mathcal{L}_{\text{align}}(\theta_1),
\end{equation}
where $\lambda_1 > 0, \lambda_2 > 0, \lambda_3 > 0$ are hyper-parameters. Here, $\cL_{\text{ce}}(f_{\theta_2}(f_{\theta_1}(x)),y)$ and $\cL_{\text{ce}}(f_{\theta_1}(x), \bm{a})$ denote the cross-entropy loss for predicting $y$ and $\bm{a}$, respectively. The alignment loss $\mathcal{L}_{\text{align}}(\theta_2)$ over $\theta_2$ is defined as
\begin{equation*}
    \mathcal{L}_{\text{align}}(\theta_2) := \frac{1}{n} \sum_{i=1}^n \left\|(a^*_i(\theta_2) - \wh{a}_i \odot (1-r_i)\right\|_{\ell_1},
    \label{eq.our loss 1}
\end{equation*}
where $\wh{a}_i:=f_{\theta_1}(x)$ and the counterfactual attribute $a^*_i(\theta_2)$ is
\begin{equation}
    a^*_i(\theta_2) = \arg\min_{a^\prime} \mathcal{L}_{\text{ce}}(f_{\theta_2}(a^\prime),y^*) + \alpha_2 {d}(a^\prime,a),
\label{eq.counter-attribute}
\end{equation}
where $y^*:=1- y$ is the counterfactual label and $a$ denotes the original attributes. Similarly, the alignment loss $\mathcal{L}_{\text{align}}(\theta_1)$ is defined in Eq.~\ref{eq.our loss}, where the counterfactual image $x^*_i(\theta_1)$ that explains the change of $\wh{a}_i$ to $a^*_i(\theta_2)$ is generated by
\begin{equation*}
    x^*_i(\theta_1) = \arg\min_{x^\prime} \mathcal{L}_{\text{ce}}(f_{\theta_1}(x^\prime),a^*) + \alpha_1 {d}(x^\prime,x).  
\label{eq.counter-image-2}
\end{equation*}
We then optimize $(\theta_1,\theta_2)$ by minimizing Eq.~\ref{eq.objective}. After optimization, our decision process $f_{\theta_2}(f_{\theta_1}(x))$ aligns well with that of the expert, with $f_{\theta_1}$ learned to employ causal imaging factors (\emph{i.e.}, $s_i \cdot x_i$) to predict causal attributes employed by $f_{\theta_2}$ to predict $y$. 


==> para/preliminary.tex <==
\section{Problem Setup \& Background}

% 1.SCM 2.identifiability of cf 3.in-distribution of cf 4.difference with AE

In this section, we introduce the problem setup and background knowledge needed to understand our work.

\textbf{Problem Setup.} We consider the classification scenario, where the system contains an image $x\in\mathcal{X}$ and a label $y\in\mathcal{Y}$ from an expert annotator. In addition to $y$, we assume the expert also provides an explanation $e$ to explain his decision of labeling $x$ as $y$. Commonly, the explanation could refer to region of interest annotation or attribute descriptions. For example, radiologists often write an \emph{annotation} section and an \emph{observation} section, which respectively describe which body part is abnormal and what phenomena are observed, in their reports to explain their diagnosis \cite{xie2020chexplain}. Motivated by this, we assume for each sample, the explanation can be formulated as a binary mask $s$ indicating the abnormal area and an attribute description $a=[a_1,...,a_p] \in \mathcal{A}$ of the abnormality. In this regard, our data can be denoted as $\mathcal{D}=\{(x_i,y_i,e_i=(s_i,a_i))\}_{i=1}^n$. With this data, \textbf{our goal} is then to learn a classifier $f_\theta: \mathcal{X}\mapsto \mathcal{Y}$ that \textbf{i)} predicts $y$ accurately \textbf{ii)} has a decision mechanism that is aligned with the radiologists.

\textbf{Counterfactual Generation (CF).} Using the counterfactual definition of causation \cite{pearl2009causality}, we can probe the causal decision mechanism of the classifier by generating the counterfactual image and observing its difference from the original. Specifically, for the sample pair $(x,y)$ and the classifier $f_\theta$, the counterfactual image $x^*$ with respect to the counterfactual class $y^*\neq y$ can be obtained\footnote{We note a recent work \cite{pan2024counterfactual} claimed unidentifiability of the counterfactual image $x^*$. To see the difference, note that they faced unidentifiability because their causal model and exogenous variables are \emph{unobservable}. However, in our case, the classifier $f_\theta$ is fixed and known, hence inducing the identification of the counterfactual image with Eq.~\ref{eq.objective.cf}.} by \cite{augustin2024dig,guyomard2023generating,verma2020counterfactual,dhurandhar2018explanations}:
\begin{equation}
    x^* = \arg\min_{x^\prime} \mathcal{L}_{\text{ce}}(f_\theta(x^\prime),y^*) + \alpha {d}(x^\prime,x),
    \label{eq.objective.cf}
\end{equation}
where $\mathcal{L}_{\text{ce}}$ is the cross-entropy loss for classification, ${d}$ is a distance metric that constrains the modification of $x$ to be sparse, and $\alpha$ is the regularization hyperparameter. In this regard, the modified area $\mathbbm{1}(\left|x^* - x\right|> 0)$ is responsible for the classification of $x$ as $y$, in that if we modified $x$ to $x^*$, the model would have made a different decision $y^*$.

To ensure the realism of the counterfactual image, we can implement Eq.~\ref{eq.objective.cf} via gradient descent in the latent space of the image. Notable, this strategy has been shown effective for generating realistic images \cite{goyal2019counterfactual,balasubramanian2020latent,zemni2023octet}, as also verified by the visualization of generated counterfactual image in Fig.~\ref{fig.visu-cf-img}.

Indeed, Eq.~\ref{eq.objective.cf} is similar to the optimization in \textbf{Adversarial Attack (AA)} \cite{szegedy2013intriguing}. However, what differentiates CF from and AA is \emph{perceptibility}. While CF provides sparse human interpretable solutions that modify only a few variables, AA usually favours making small changes to many variables for imperceptibility \cite{wachter2017counterfactual}. This often leads to different choices of the distance function $d$ and the hyperparameter $\alpha$ \cite{freiesleben2022intriguing,guidotti2024counterfactual}.




==> para/preliminary_xw_v1.tex <==
\section{Problem Setup \& Background}

% 1.SCM 2.identifiability of cf 3.in-distribution of cf 4.difference with AE

In this section, we formulate our problem and introduce the background knowledge. 

\textbf{Problem Setup.} We consider the classification scenario, where the system contains an image $x\in\mathcal{X}$ and a label $y\in\mathcal{Y}$ from an expert annotator. In addition to $y$, we assume the expert also provides an explanation $e$ to explain his decision of labeling $x$ as $y$. Commonly, the explanation could refer to region of interest annotation or attribute descriptions. For example, radiologists often write an \emph{annotation} section and an \emph{observation} section, which respectively describe which body part is abnormal and what phenomena are observed, in their reports to explain their diagnosis \cite{xie2020chexplain}. Motivated by this, we assume for each sample, the explanation can be formulated as a binary mask $s$ indicating the abnormal area, along with a binary attribute description $a=[a_1,...,a_p] \in \mathcal{A}$ of the abnormality. In this regard, our data can be denoted as $\mathcal{D}=\{(x_i,y_i,e_i=(s_i,a_i))\}_{i=1}^n$. With this data, \textbf{our goal} is then to learn a classifier $f_\theta: \mathcal{X}\mapsto \mathcal{Y}$ that \textbf{i)} predicts $y$ accurately \textbf{ii)} has a decision mechanism that is aligned with the radiologists.


\textbf{Counterfactual analysis and Cause of Effect.} Different from the ``effect of cause" (\emph{e.g.} average treatment effect) that measures the effect of an treatment towards an outcome, the goal of ``cause of effect" is to measure the likelihood that one event was an cause of another. For this purpose, \cite{pearl2009causality} defines the following counterfactual quantity called \emph{probability of causation}: 
\begin{equation}
\label{eq.coe}
    \mathbb{P}(Y_{x^\prime} = y^\prime|X=x,Y=y), 
\end{equation}
which reads as ``the probability of $Y$ would be $y^\prime$ had $X$ been $x^\prime$ if we factually observed that $Y=y$ and $X=x$"\footnote{Under the \emph{exogeneity} and \emph{monotonicity} conditions for binary $X,Y$, Eq.~\ref{eq.coe} is identifiable.}. Here, $Y_x$ denotes the unit-counterfactual \cite{pearl2009causal} or potential outcome. IN our scenario, rather than considering the whole image $x$, we are looking for specific regions within the image that causally determines the radiologist's decision. To achieve this, we first probe the classifier's decision mechanism via counterfactual generation. 

% In our medical scenario, $X$ is a high-dimensional image, where only a certain region may be the cause of the disease label. To identify such a causal region, 

\textbf{Counterfactual Generation (CF).} Given a classifier $f_\theta$ and any sample $(x,y)$, CF generates a counterfactual image $x^*$ with respect to the counterfactual class $y^*\neq y$ that can be obtained by \cite{augustin2024dig,guyomard2023generating,verma2020counterfactual,dhurandhar2018explanations}: 
%Using the counterfactual definition of causation \cite{pearl2009causality}, we can probe the causal decision mechanism of the classifier by generating the counterfactual image and observing its difference from the original. Specifically, for the sample pair $(x,y)$ and the classifier $f_\theta$, the counterfactual image $x^*$ with respect to the counterfactual class $y^*\neq y$ can be obtained\footnote{We note a recent work \cite{pan2024counterfactual} claimed unidentifiability of the counterfactual image $x^*$. To see the difference, note that they faced unidentifiability because their causal model and exogenous variables are \emph{unobservable}. However, in our case, the classifier $f_\theta$ is fixed and known, hence inducing the identification of the counterfactual image with Eq.~\ref{eq.objective.cf}.} by \cite{augustin2024dig,guyomard2023generating,verma2020counterfactual,dhurandhar2018explanations}:
\begin{equation}
    x^* = \arg\min_{x^\prime} \mathcal{L}_{\text{ce}}(f_\theta(x^\prime),y^*) + \alpha {d}(x^\prime,x),
    \label{eq.objective.cf}
\end{equation}
where $\mathcal{L}_{\text{ce}}$ is the cross-entropy loss for classification, ${d}$ is a distance metric that constrains the modification of $x$ to be sparse, and $\alpha$ is the regularization hyperparameter. In this regard, the modified area $\mathbbm{1}(\left|x^* - x\right|> 0)$ is responsible for the classification of $x$ as $y$, in that if we modified $x$ to $x^*$, the model would have made a different decision $y^*$. In Appx.~\ref{appx.theory}, we show that if $d(\cdot,x)$ is convex and $x^*$ is unique, then $x^*$ maximizes $\max_{d(x^\prime,x)\leq d_\alpha} \mathbb{P}_\theta(Y_{x^\prime} = y^\prime|X=x,Y=y)$ for some $\alpha$\footnote{This term is identifiable since $f_\theta$ is known (see Prop.~\ref{prop.identify} in the appendix for details).}, where $\mathbb{P}_\theta(Y_{x^\prime} = y^\prime|X=x,Y=y)$ is induced by the classifier's parameter $\theta$. 


% \footnote{We note a recent work \cite{pan2024counterfactual} claimed unidentifiability of the counterfactual image $x^*$. To see the difference, note that they faced unidentifiability because their causal model and exogenous variables are \emph{unobservable}. However, in our case, the classifier $f_\theta$ is fixed and known, hence inducing the identification of the counterfactual image with Eq.~\ref{eq.objective.cf}.}

To ensure the realism of the counterfactual image, we can implement Eq.~\ref{eq.objective.cf} via gradient descent in the latent space of the image. Notable, this strategy has been shown effective for generating realistic images \cite{goyal2019counterfactual,balasubramanian2020latent,zemni2023octet}, as also verified by the visualization of generated counterfactual image in Fig.~\ref{fig.visu-cf-img}.

Indeed, Eq.~\ref{eq.objective.cf} is similar to but different from the optimization in \textbf{Adversarial Attack (AA)} \cite{szegedy2013intriguing} concerning \emph{perceptibility}. Although both methods share the same objective framework, CF aims at highlighting significant areas that explain the classifier's decision process while AA favours making small and imperceptible changes to alter the prediction outcome \cite{wachter2017counterfactual}. This often leads to different choices of the distance function $d$ and the hyperparameter $\alpha$ \cite{freiesleben2022intriguing,guidotti2024counterfactual}.

% CF provides sparse human interpretable solutions that modify only a few variables, 


==> para/related_works.tex <==
\section{Related Works}

\textbf{Visual Alignment.} Alignment is more broadly studied in natural language processing \cite{ouyang2022training}, reinforcement learning \cite{ibarz2018reward}, and value-driven learning \cite{al2024training}. In the realm of visual alignment, \cite{hind2019ted,rieger2020interpretations} proposed to align the decision basis of deep learning models with human by simultaneously predicting the class label and the decision area. \cite{zhang2018interpretable,liu2021act,muller2023anatomy} aligned the decision-making process of neural networks by incorporating expert knowledge into architecture design. Of particular relevance to our work are \cite{ross2017right,gao2022aligning,zhang2023magi}, who suggested constraining the input image gradient to be significant in areas annotated by experts. However, the input gradient can be biased by pseudo-correlations that exist between expert features and shortcut features \cite{geirhos2020shortcut}, leading to a misaligned model. In contrast, we adopt counterfactual generation to identify the causal areas that drive the model's decision-making. By ensuring these factors are confined to expert-annotated areas, our model can effectively learn an expert-aligned decision-making process.

\textbf{Explaining Medical AI.} Explainability is essential for physicians to trust and effectively utilize the results generated by medical diagnosis models \cite{lipton2017doctor}. To address this need, various explanation techniques have been developed \cite{wani2024explainable}. For example, \emph{attribution-based methods} explain model predictions by assessing the importance of different features \cite{suryani2022lung,yuen2024tutorial}. \emph{Example-based methods} utilize similar images \cite{barnett2021interpretable} or prototypes \cite{gallee2024evaluating} to interpret the underlying decision rules. Additionally, \emph{text-based explanations} provide image captions that effectively communicate the rationale behind decisions to radiologists \cite{zhang2017mdnet,singh2019chest,reale2024vision}. However, these approaches focus on interpreting models that have been trained. If misalignment occurs during the training process, their utility can be limited. In contrast, we propose an alignment loss to learn an intrinsically explainable model.


==> para/related_works_xw_v1.tex <==
\section{Related Works}

\textbf{Learning Visual Alignment.} Alignment is broadly studied in natural language processing \cite{ouyang2022training} and reinforcement learning \cite{ibarz2018reward}. In the realm of visual alignment, \cite{hind2019ted,rieger2020interpretations} proposed to align deep learning models with humans by simultaneously predicting the class label and the decision area. \cite{zhang2018interpretable,liu2021act,muller2023anatomy} aligned the decision-making process of neural networks by incorporating expert knowledge into architecture design. Of particular relevance to our work are \cite{ross2017right,gao2022aligning,zhang2023magi}, which suggested constraining the input image gradient to be significant in areas annotated by experts. However, the input gradient can be biased by pseudo-correlations that exist between expert features and shortcut features \cite{geirhos2020shortcut}, leading to a misaligned model. In contrast, we adopt counterfactual generation to identify causal areas that determine the model's prediction. By ensuring these factors are confined to expert-annotated areas, our model can be effectively aligned with expert's decision-process. 


\textbf{Explaining Medical AI.} Explainability is essential for physicians to trust and effectively utilize the results generated by medical diagnosis models \cite{lipton2017doctor}. To fulfill this requirement, various explanation techniques have been developed \cite{wani2024explainable}. For example, \emph{attribution-based methods} explained model predictions by assessing the importance of different features \cite{suryani2022lung,yuen2024tutorial}. \emph{Example-based methods} utilized similar images \cite{barnett2021interpretable} or prototypes \cite{gallee2024evaluating} to interpret the underlying decision rules. Additionally, \emph{text-based explanations} provided image captions that effectively communicate the rationale behind decisions to radiologists \cite{zhang2017mdnet,singh2019chest,reale2024vision}. However, these approaches focused on interpreting models that have been trained. If misalignment occurs during the training process, their utility could be limited. In contrast, we propose causal alignment to learn an intrinsically explainable model.

